Bring Your Own Knowledge: A Survey of Methods for LLM Knowledge Expansion

Adapting large language models (LLMs) to new and diverse knowledge is essential for their lasting effectiveness in real-world applications. This survey provides an overview of state-of-the-art methods for expanding the knowledge of LLMs, focusing on integrating various knowledge types, including factual information, domain expertise, language proficiency, and user preferences. We explore techniques, such as continual learning, model editing, and retrieval-based explicit adaptation, while discussing challenges like knowledge consistency and scalability. Designed as a guide for researchers and practitioners, this survey sheds light on opportunities for advancing LLMs as adaptable and robust knowledge systems.

==> taxonomy.tex <==
\tikzset{
    every node/.style={
        align=left,
    }
}
\begin{figure*}[ht]
\centering
\resizebox{\textwidth}{!}{
    \begin{forest}
    for tree={
        text width=3.5cm,
        grow=east,
        parent anchor=east,
        child anchor=west,
        anchor=center,
        rounded corners,
        font=\footnotesize,
        edge={thick},
        forked edges,
        draw,
        l sep=5mm
    }
    [Knowledge Expansion Methods,
        rotate=90,
        text width=4.2cm,
        draw=gray!50, 
        line width=0.5mm, 
        fill=gray!20,
        [
            Retrieval-based Methods (§\ref{sec:retrieval}), 
            text width=4.0cm,
            draw=yellow!50, 
            line width=0.5mm, 
            fill=yellow!20
            [
                Domain Adaptation (§\ref{sec:retrieval-domain}),
                text width=5.1cm,
                draw=yellow!50, 
                line width=0.5mm, 
                fill=yellow!20,
            ]
            [
                Updating Facts (§\ref{sec:retrieval-facts}),
                text width=5.1cm,
                draw=yellow!50, 
                line width=0.5mm, 
                fill=yellow!20,
            ]
        ]
        [
            Model Editing (§\ref{sec:model-editing}), 
            text width=4.0cm,
            draw=red!50, 
            line width=0.5mm, 
            fill=red!20 
            [
                Updating Preferences (§\ref{sec:model-editing-preference}), 
                text width=5.1cm,
                draw=red!50, 
                line width=0.5mm, 
                fill=red!20,
            ]
            [
                Updating Facts (§\ref{sec:model-editing-facts}), 
                text width=5.1cm,
                draw=red!50, 
                line width=0.5mm,
                fill=red!20,
            ] 
        ]
        [
            Continual Learning (§\ref{sec:continual-learning}), 
            text width=4.0cm,
            draw=orange!50, 
            line width=0.5mm, 
            fill=orange!20 
            [
                Continual Preference Alignment (§\ref{sec:continual-alignment}), 
                text width=5.1cm,
                draw=orange!50, 
                line width=0.5mm, 
                fill=orange!20,
            ]
            [
                Continual Pretraining, 
                text width=5.1cm,
                draw=orange!50, 
                line width=0.5mm, 
                fill=orange!20, 
                [
                    Language Expansion (§\ref{sec:continual-pretraining-language}),
                    text width=4.2cm,
                    draw=orange!50, 
                    line width=0.5mm, 
                    fill=orange!20,
                    [
                        Programming Language,
                        text width=3.2cm,
                        draw=orange!50, 
                        line width=0.5mm, 
                        fill=orange!20,
                    ]
                    [
                        Natural Language,
                        text width=3.2cm,
                        draw=orange!50, 
                        line width=0.5mm, 
                        fill=orange!20,
                    ]
                ]
                [
                    Domain Adaptation (§\ref{sec:continual-pretraining-domain}),
                    text width=4.2cm,
                    draw=orange!50, 
                    line width=0.5mm, 
                    fill=orange!20,
                ]
                [
                    Updating Facts (§\ref{sec:continual-pretraining-facts}),
                    text width=4.2cm,
                    draw=orange!50, 
                    line width=0.5mm, 
                    fill=orange!20, 
                ],
            ] 
        ]
    ]
    \end{forest}
}
\caption{Taxonomy of current methods for expanding LLM knowledge. Due to space constraints, please refer to Appendix \ref{sec:appendix_taxonomy} for a comprehensive review of methods and their corresponding citations.}
\label{fig:taxonomy}
\end{figure*}
